The PEPSI Exoplanet Transit Survey. III: The detection of FeI, CrI and TiI in the atmosphere of MASCARA-1 b through high-resolution emission spectroscopy

Hot giant planets like MASCARA-1 b are expected to have thermally inverted atmospheres, that makes them perfect laboratory for the atmospheric characterization through high-resolution spectroscopy. Nonetheless, previous attempts of detecting the atmosphere of MASCARA-1 b in transmission have led to negative results. In this paper we aim at the detection of the optical emission spectrum of MASCARA-1 b. We used the high-resolution spectrograph PEPSI to observe MASCARA-1 (spectral type A8) near the secondary eclipse of the planet. We cross-correlated the spectra with synthetic templates computed for several atomic and molecular species. We obtained the detection of FeI, CrI and TiI in the atmosphere of MASCARA-1 b with a S/N ~7, 4 and 5 respectively, and confirmed the expected systemic velocity of ~13 km/s and the radial velocity semi-amplitude of MASCARA-1 b of ~200 km/s. The detection of Ti is of particular importance in the context of the recently proposed Ti cold-trapping below a certain planetary equilibrium temperature. We confirm the presence of an the atmosphere around MASCARA-1 b through emission spectroscopy. We conclude that the atmospheric non detection in transmission spectroscopy is due to the high gravity of the planet and/or to the overlap between the planetary track and its Doppler shadow.

==> previous.tex <==
\section{Previous works {\bf TO BE REMOVED IN THE FINAL VERSION}}

